Study of X-ray emission from the S147 nebula by SRG/eROSITA: supernova-in-the-cavity scenario

The Simeis~147 nebula (S147), particularly well known for a spectacular net of ${\rm H}_\alpha$-emitting filaments, is often considered one of the largest and oldest known supernova remnants in the Milky Way. Here, and in a companion paper, we present studies of X-ray emission from the S147 nebula using the data of SRG/eROSITA All-Sky Survey observations. In this paper, we argue that many inferred properties of the X-ray emitting gas are broadly consistent with a scenario of the supernova explosion in a low-density cavity, e.g. a wind-blown-bubble. This scenario assumes that a $\sim 20\,{\rm M_\odot}$ progenitor star has had small velocity with respect to the ambient ISM, so it stayed close to the center of a dense shell created during its Main Sequence evolution till the moment of the core-collapse explosion. The ejecta first propagate through the low-density cavity until they collide with the dense shell, and only then the reverse shock goes deeper into the ejecta and powers the observed X-ray emission of the nebula. The part of the remnant inside the dense shell remains non-radiative till now and, plausibly, in a state with $T_e<T_i$ and Non-Equilibrium Ionization (NEI). On the contrary, the forward shock becomes radiative immediately after entering the dense shell, and, being subject to instabilities, creates a characteristic "foamy" appearance of the nebula in ${\rm H}_\alpha$ and radio emission.

==> notes.tex <==
narrow bands : (300-440),440-620, 620-800, 800-1100,(1100-1400, 1400-2100)
